Pentimento: Data Remanence in Cloud FPGAs

Cloud FPGAs strike an alluring balance between computational efficiency, energy efficiency, and cost. It is the flexibility of the FPGA architecture that enables these benefits, but that very same flexibility that exposes new security vulnerabilities. We show that a remote attacker can recover "FPGA pentimenti" - long-removed secret data belonging to a prior user of a cloud FPGA. The sensitive data constituting an FPGA pentimento is an analog imprint from bias temperature instability (BTI) effects on the underlying transistors. We demonstrate how this slight degradation can be measured using a time-to-digital (TDC) converter when an adversary programs one into the target cloud FPGA. This technique allows an attacker to ascertain previously safe information on cloud FPGAs, even after it is no longer explicitly present. Notably, it can allow an attacker who knows a non-secret "skeleton" (the physical structure, but not the contents) of the victim's design to (1) extract proprietary details from an encrypted FPGA design image available on the AWS marketplace and (2) recover data loaded at runtime by a previous user of a cloud FPGA using a known design. Our experiments show that BTI degradation (burn-in) and recovery are measurable and constitute a security threat to commercial cloud FPGAs.

==> figs/AES_arch.tex <==
\begin{figure}[!htb]
\begin{subfigure}[t]{\linewidth}
  \centering
  \includegraphics[width=\linewidth]{src/AES_arch.pdf}
\end{subfigure}
\caption{\cd{This shows how simple physical separation can create long routes containing critical information}}
\label{fig/AES_arch}
\end{figure} 

==> figs/BTI.tex <==
\begin{figure}
    \centering
    \begin{subfigure}
        \centering
        \includegraphics[width=\linewidth]{src/PMOS_NBTI.pdf}
        \caption{PMOS NBTI}
        \label{fig/transistor_model/PMOS_NBTI}
    \end{subfigure}
        \begin{subfigure}
        \centering
        \includegraphics[width=\linewidth]{src/PMOS_NBTI.pdf}
        \caption{\cd{todo NMOS NBTI}}
        \label{fig/transistor_model/NMOS_NBTI}
    \end{subfigure}
\caption[\cd{TODO redo}Simplified cross sectional view of NMOS and PMOS transistors and degradation mechanisms.]{Simplified cross sectional view of NMOS and PMOS transistors and degradation mechanisms. (a) and (b) depicts unaffected NMOS and PMOS architectures. (c) depicts a PMOS device affected by Negative Bias Temperature Instability (NBTI). (d) depicts a PMOS device affected by Hot Carrier Injection (HCI). Finally, (e) depicts a PMOS device affected by Time Dependent Dielectric Breakdown (TDDB).} 
\label{fig/transistor_model}
\end{figure}


==> figs/burnin_measurement_schedule.tex <==
\begin{figure*}[!htb]
\begin{subfigure}
  \centering
  \includegraphics[width=\linewidth]{src/burnin_measurement_schedule.pdf}
\end{subfigure}
\caption[This figure depicts 3 hours of the \textit{Burn-in/Measurement} phase of our experiment, and a high level view of the designs used.]{This figure presents 3 hours of the \textit{Burn-in/Measurement} phase of our experiment, and a high level view of the designs used. The \textit{Measure} design contains a set of tested nets which we wish to observe the burn-in effect on, and a \texttt{Carry Chain} for each of these nets. The Burn-in design initializes these same test nets with a fixed value, VCC (logical 1 value) or GND (logical 0 value), and increases internal temperature with \texttt{DSP Power Wasters}. Short periods of measurement taking $\delta$ time are interleaved with periods of 60 minute burn-in stress with the \textit{Burn-in} design.}
\label{fig/burnin_measurement_schedule}
\end{figure*}

==> figs/experiment_1_schedule.tex <==
\newcommand{\STAB}[1]{\begin{tabular}{@{}c@{}}#1\end{tabular}}
\begin{table*}[ht!]
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
Hour & \STAB{\rotatebox[origin=c]{90}{\;[$-\delta$,0)\;}} & \STAB{\rotatebox[origin=c]{90}{\;[0,$\delta$]\;}} & \STAB{\rotatebox[origin=c]{90}{\;($\delta$,1)\;}} & \STAB{\rotatebox[origin=c]{90}{\;[1,1+$\delta$]\;}} & \STAB{\rotatebox[origin=c]{90}{\;(1+$\delta$,2)\;}} & \STAB{\rotatebox[origin=c]{90}{\;[2, 2+$\delta$]\;}} & \STAB{\rotatebox[origin=c]{90}{\;(2,200)\;}} & \STAB{\rotatebox[origin=c]{90}{\;[200, 200+$\delta$]\;}} & \STAB{\rotatebox[origin=c]{90}{\;(200+$\delta$,201)\;}} & \STAB{\rotatebox[origin=c]{90}{\;[201, 201+$\delta$]\;}} & \STAB{\rotatebox[origin=c]{90}{\;(202+$\delta$,202)\;}} & \STAB{\rotatebox[origin=c]{90}{\;[202,202+$\delta$]\;}} & \STAB{\rotatebox[origin=c]{90}{\;(202,400]\;}} \\ \hline
Architecture  & \STAB{\rotatebox[origin=c]{90}{\;Calibrate\;}} & \STAB{\rotatebox[origin=c]{90}{\;Measure\;}} & \STAB{\rotatebox[origin=c]{90}{\;Burn-in\;}} & \STAB{\rotatebox[origin=c]{90}{\;Measure\;}} & \STAB{\rotatebox[origin=c]{90}{\;Burn-in\;}} & \STAB{\rotatebox[origin=c]{90}{\;Measure\;}} & \dots & \STAB{\rotatebox[origin=c]{90}{\;Measure\;}} & \STAB{\rotatebox[origin=c]{90}{\;Burn-in\;}} & \STAB{\rotatebox[origin=c]{90}{\;Measure\;}} & \STAB{\rotatebox[origin=c]{90}{\;Burn-in\;}} & \STAB{\rotatebox[origin=c]{90}{\;Measure\;}} & \dots \\ \hline
Burn Value & --- & ---  & $x$ & ---  & $x$  & --- & --- & --- & $\overline{x}$ & --- & $\overline{x}$ & --- & --- \\ \hline
\end{tabular}
\vspace{10px}
\caption{Experiment 1 schedule}
\end{table*}


==> figs/experiment_2_schedule.tex <==
\newcommand{\STAB}[1]{\begin{tabular}{@{}c@{}}#1\end{tabular}}
\begin{table*}[ht!]
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
Hour & \STAB{\rotatebox[origin=c]{90}{\;[$-\delta$,0)\;}} & \STAB{\rotatebox[origin=c]{90}{\;[0,$\delta$]\;}} & \STAB{\rotatebox[origin=c]{90}{\;($\delta$,1)\;}} & \STAB{\rotatebox[origin=c]{90}{\;[1,1+$\delta$]\;}} & \STAB{\rotatebox[origin=c]{90}{\;(1+$\delta$,2)\;}} & \STAB{\rotatebox[origin=c]{90}{\;[2, 2+$\delta$]\;}} & \STAB{\rotatebox[origin=c]{90}{\;(2,200)\;}} & \STAB{\rotatebox[origin=c]{90}{\;[200, 200+$\delta$]\;}} & \STAB{\rotatebox[origin=c]{90}{\;(200+$\delta$,201)\;}} & \STAB{\rotatebox[origin=c]{90}{\;[201, 201+$\delta$]\;}} & \STAB{\rotatebox[origin=c]{90}{\;(202+$\delta$,202)\;}} & \STAB{\rotatebox[origin=c]{90}{\;[202,202+$\delta$]\;}} & \STAB{\rotatebox[origin=c]{90}{\;(202,400]\;}} \\ \hline
Architecture  & \STAB{\rotatebox[origin=c]{90}{\;Calibrate\;}} & \STAB{\rotatebox[origin=c]{90}{\;Measure\;}} & \STAB{\rotatebox[origin=c]{90}{\;Burn-in\;}} & \STAB{\rotatebox[origin=c]{90}{\;Measure\;}} & \STAB{\rotatebox[origin=c]{90}{\;Burn-in\;}} & \STAB{\rotatebox[origin=c]{90}{\;Measure\;}} & \dots & \STAB{\rotatebox[origin=c]{90}{\;Measure\;}} & \STAB{\rotatebox[origin=c]{90}{\;Burn-in\;}} & \STAB{\rotatebox[origin=c]{90}{\;Measure\;}} & \STAB{\rotatebox[origin=c]{90}{\;Burn-in\;}} & \STAB{\rotatebox[origin=c]{90}{\;Measure\;}} & \dots \\ \hline
Burn Value & --- & ---  & $x$ & ---  & $x$  & --- & --- & --- & $\overline{x}$ & --- & $\overline{x}$ & --- & --- \\ \hline
\end{tabular}
\vspace{10px}
\caption{Experiment 1 schedule}
\end{table*}


==> figs/opentitan_block_diagram.tex <==
\begin{figure}[!htb]
\begin{subfigure}[t]{\linewidth}
  \centering
  \includegraphics[width=\linewidth]{src/top_earlgrey_block_diagram_august_2022.pdf}
\end{subfigure}
\caption[]{The block-level diagram of the OpenTitan Earl Grey chip. This architectural description is a production of the OpenTitan project\footnotemark.}
\label{fig/opentitan_block_diagram}
\end{figure} 

==> figs/opentitan_route_hist.tex <==
\begin{figure}[!htb]
\centering
\begin{subfigure}[t]{\linewidth}
    \centering
    \includegraphics[width=\linewidth]{src/ot_route_delay_hist_combined.pdf}
    \caption{}
    \label{fig/ot_hist_sep}
\end{subfigure}
\begin{subfigure}[t]{\linewidth}
    \centering
    \includegraphics[width=\linewidth]{src/ot_route_delay_hist_separated.pdf}
    \caption{}
    \label{fig/ot_hist_com}
\end{subfigure}
\caption{(a) The distribution of route lengths (in ps) for a selection of twenty security-critical assets in an OpenTitan Earl Grey implemented on a Virtex UltraScale+. (b) The distribution of route lengths (in ps) for the top five security-critical assets with respect to mean route length. Refer to Table~\ref{table/ot_hist_table} for more information.} 
\label{fig/ot_hist}
\vspace{-15px}
\end{figure} 


==> figs/route_dist.tex <==
\begin{figure}[!htb]
\begin{subfigure}[t]{\linewidth}
  \centering
  %\includegraphics[width=\linewidth]{src/AES_arch.pdf}
\end{subfigure}
\caption{\cd{show that AES routes are within reason for measurement}}
\label{fig/aes_route_dist}
\end{figure} 

==> src/docs/29676d62-aca6-4694-a7f2-b84d8b38bcbe <==
{"id":"r0.049527695018553364","lines":[{"id":"n0.9671014379546016","blocks":[]},{"id":"n0.564236306069992","blocks":[{"id":"n0.030955479974488442","text":"\\diagram","type":"composite","elements":{"de18503309665940448":{"id":"de18503309665940448","lines":[{"blocks":[{"id":"n0.30121449018753865","text":"Measure"}],"id":"n0.6526306742982805"}],"shape":{"data":{"p":{"x":128.84645850033007,"y":7.451535133837851},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false},"de9832369207353053":{"id":"de9832369207353053","lines":[{"id":"n0.7243417646641581","blocks":[{"id":"n0.40238834817736335","text":"Test ","style":{"fontSize":"\\small"}}],"style":{"lineHeightEm":0.7,"align":"center"}},{"id":"n0.1712013747772897","blocks":[{"id":"n0.0644576382047698","text":"Routes"}],"style":{"lineHeightEm":0.7,"align":"center"}}],"shape":{"data":{"p":{"x":153.29441223188377,"y":188.597235252389},"rotation":0},"anchor":"center"},"isTextMode":true,"isInGroup":false},"de6719266961223402":{"id":"de6719266961223402","lines":[{"id":"n0.11744846719008628","blocks":[{"id":"n0.03871968741653631","text":"Pulse","style":{"fontSize":"\\small"}}],"style":{"lineHeightEm":0.7,"textDirection":"rtl","align":"center"}},{"id":"n0.38316976370998124","blocks":[{"id":"n0.9325747081748399","text":"Generator","style":{"fontSize":"\\small"}}],"style":{"lineHeightEm":0.7,"textDirection":"rtl","align":"center"}}],"shape":{"data":{"p":{"x":49.22880377020125,"y":264.40721217953154},"rotation":0},"anchor":"center"},"isTextMode":true,"isInGroup":false},"de23150534795523248":{"id":"de23150534795523248","lines":[{"id":"n0.3911430741393178","blocks":[{"id":"n0.18919973813424373","text":"Carry","style":{"fontSize":"\\small"}}],"style":{"lineHeightEm":0.7,"align":"center"}},{"id":"n0.8962844622296121","blocks":[{"id":"n0.06909932784421657","text":"Chains","style":{"fontSize":"\\small"}}],"style":{"lineHeightEm":0.7,"align":"center"}}],"shape":{"data":{"p":{"x":132.37316714173411,"y":76.18256413131091},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":false}},"connections":[],"intersections":{"id":"di2581903923790777","items":[],"style":{}},"shapes":[{"id":"dp7185662901760861","type":"rectangle","data":{"p1":{"x":5.01666259765625,"y":5.850006103515625},"p2":{"x":305.01666259765625,"y":287.1000061035156}},"style":{"fillColor":"none"}},{"id":"dp2862287415152651","type":"rectangle","data":{"p1":{"x":29.33053146190323,"y":33.964964434111536},"p2":{"x":49.59206636391533,"y":146.42479775649517}}},{"id":"dp2098369552712258","type":"rectangle","data":{"p1":{"x":24.17302164220258,"y":154.45764299380826},"p2":{"x":284.99452400412474,"y":224.74503882029802}},"style":{"strokeType":".","strokeColor":[0,0,0,1],"fillColor":[0,0,255,0.4]}},{"id":"da630267659117454","data":[{"x":39.645483646723385,"y":146.42479775649517},{"x":39.645483646723385,"y":227.7573557842904}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":3}},{"id":"dp4678607490663309","type":"generic-shape","data":{"p1":{"x":90.11520362252068,"y":259.88873673354294},"p2":{"x":111.29772964818446,"y":271.93800458951256}},"subType":"pulse-1","style":{"thickness":3}},{"id":"dp5062321637531952","type":"generic-shape","data":{"p1":{"x":111.29772964818446,"y":259.88873673354294},"p2":{"x":132.48025567384823,"y":271.93800458951256}},"subType":"pulse-1","style":{"thickness":3}},{"id":"dp4657469484165868","type":"rectangle","data":{"p1":{"x":9.079210307719393,"y":246.83536322290908},"p2":{"x":89.37839723268311,"y":281.97906113615403}}},{"id":"dp7139782873624675","type":"rectangle","data":{"p1":{"x":17.173597029779742,"y":29.948541815454973},"p2":{"x":294.9411067213167,"y":154.45764299380826}},"style":{"strokeType":".","fillColor":[255,0,0,0.4]}},{"id":"da6635088931935963","data":[{"x":39.645483646723385,"y":227.7573557842904},{"x":273.942765429467,"y":227.7573557842904}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":3}},{"id":"da8592853128166283","data":[{"x":132.48025567384823,"y":271.93800458951256},{"x":151.26824525076634,"y":271.93800458951256}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":3}},{"id":"da18519585884453127","data":[{"x":150.75,"y":228},{"x":151.26824525076634,"y":271.93800458951256}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":3}},{"id":"da6895863517814381","data":[{"x":66.16970422590191,"y":145.420692101831},{"x":66.16970422590191,"y":226.7532501296263}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":3}},{"id":"da9208321138485499","data":[{"x":94.90427652001198,"y":146.42479775649517},{"x":94.90427652001198,"y":227.7573557842904}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":3}},{"id":"da557273460718351","data":[{"x":121.4284970991905,"y":146.42479775649517},{"x":121.4284970991905,"y":227.7573557842904}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":3}},{"id":"da7466946518298461","data":[{"x":192.1597519769999,"y":146.42479775649517},{"x":192.1597519769999,"y":227.7573557842904}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":3}},{"id":"da05802621945942954","data":[{"x":218.68397255617842,"y":145.420692101831},{"x":218.68397255617842,"y":226.7532501296263}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":3}},{"id":"da5836064543843619","data":[{"x":247.4185448502885,"y":146.42479775649517},{"x":247.4185448502885,"y":227.7573557842904}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":3}},{"id":"da2887600822175409","data":[{"x":273.942765429467,"y":146.42479775649517},{"x":273.942765429467,"y":227.7573557842904}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":3}},{"id":"da8724238546064775","data":[{"x":142.05846892341197,"y":40.99370401676051},{"x":168.95105897021867,"y":40.99370401676051}],"head":"no","tail":"no","shaft":".","mVer":1},{"id":"da7171589231179621","data":[{"x":142.05846892341197,"y":67.10045103802813},{"x":168.95105897021867,"y":67.10045103802813}],"head":"no","tail":"no","shaft":".","mVer":1},{"id":"da6890158277566706","data":[{"x":142.05846892341197,"y":115.29752246190682},{"x":168.95105897021867,"y":115.29752246190682}],"head":"no","tail":"no","shaft":".","mVer":1},{"id":"da019845227921771125","data":[{"x":142.05846892341197,"y":137.38784686451788},{"x":168.95105897021867,"y":137.38784686451788}],"head":"no","tail":"no","shaft":".","mVer":1},{"id":"da6550864989106079","data":[{"x":140.95329306594618,"y":167.51101650444207},{"x":167.84588311275292,"y":167.51101650444207}],"head":"no","tail":"no","shaft":".","mVer":1},{"id":"da5379769768317879","data":[{"x":140.95329306594618,"y":210.68755965500006},{"x":167.84588311275292,"y":210.68755965500006}],"head":"no","tail":"no","shaft":".","mVer":1},{"id":"da986732709781526","data":[{"x":28.59372507206567,"y":49.02654925407362},{"x":37.43513193179184,"y":49.02654925407362},{"x":49.59206636391533,"y":49.02654925407362}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da48594373154144965","data":[{"x":28.59372507206567,"y":63.08402841937157},{"x":49.59206636391533,"y":63.08402841937157}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da5965278670167868","data":[{"x":28.59372507206567,"y":77.14150758466953},{"x":49.59206636391533,"y":77.14150758466953}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da5839147143297054","data":[{"x":28.59372507206567,"y":91.19898674996747},{"x":49.59206636391533,"y":91.19898674996747}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da673191056114586","data":[{"x":28.59372507206567,"y":105.25646591526542},{"x":49.59206636391533,"y":105.25646591526542}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da24387463045406055","data":[{"x":28.59372507206567,"y":119.31394508056339},{"x":49.59206636391533,"y":119.31394508056339}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da6871682958087638","data":[{"x":29.69890092953144,"y":132.36731859119718},{"x":50.69724222138111,"y":132.36731859119718}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"dp3822830385639815","type":"rectangle","data":{"p1":{"x":55.85475204108176,"y":33.964964434111536},"p2":{"x":76.11628694309385,"y":146.42479775649517}}},{"id":"da21948554331900527","data":[{"x":55.11794565124419,"y":49.02654925407362},{"x":63.95935251097037,"y":49.02654925407362},{"x":76.11628694309385,"y":49.02654925407362}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da40556812144745424","data":[{"x":55.11794565124419,"y":63.08402841937157},{"x":76.11628694309385,"y":63.08402841937157}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da5030493778323746","data":[{"x":55.11794565124419,"y":77.14150758466953},{"x":76.11628694309385,"y":77.14150758466953}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da11165610456036978","data":[{"x":55.11794565124419,"y":91.19898674996747},{"x":76.11628694309385,"y":91.19898674996747}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da6353185792535332","data":[{"x":55.11794565124419,"y":105.25646591526542},{"x":76.11628694309385,"y":105.25646591526542}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da7496403721312409","data":[{"x":55.11794565124419,"y":119.31394508056339},{"x":76.11628694309385,"y":119.31394508056339}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da6043445533023242","data":[{"x":56.223121508709966,"y":132.36731859119718},{"x":77.22146280055962,"y":132.36731859119718}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"dp6087682667174085","type":"rectangle","data":{"p1":{"x":84.58932433519183,"y":33.964964434111536},"p2":{"x":104.85085923720393,"y":146.42479775649517}}},{"id":"da44026055280543985","data":[{"x":83.85251794535426,"y":49.02654925407362},{"x":92.69392480508044,"y":49.02654925407362},{"x":104.85085923720393,"y":49.02654925407362}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da6424273540848545","data":[{"x":83.85251794535426,"y":63.08402841937157},{"x":104.85085923720393,"y":63.08402841937157}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da27611474538144165","data":[{"x":83.85251794535426,"y":77.14150758466953},{"x":104.85085923720393,"y":77.14150758466953}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da883688770776955","data":[{"x":83.85251794535426,"y":91.19898674996747},{"x":104.85085923720393,"y":91.19898674996747}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da01333746172489969","data":[{"x":83.85251794535426,"y":105.25646591526542},{"x":104.85085923720393,"y":105.25646591526542}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da44784794097669134","data":[{"x":83.85251794535426,"y":119.31394508056339},{"x":104.85085923720393,"y":119.31394508056339}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da8262953373980814","data":[{"x":84.95769380282003,"y":132.36731859119718},{"x":105.9560350946697,"y":132.36731859119718}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"dp06909276142612708","type":"rectangle","data":{"p1":{"x":112.21872077183612,"y":33.964964434111536},"p2":{"x":132.48025567384823,"y":146.42479775649517}}},{"id":"da7851162831452594","data":[{"x":111.48191438199856,"y":49.02654925407362},{"x":120.32332124172473,"y":49.02654925407362},{"x":132.48025567384823,"y":49.02654925407362}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da7383504134853426","data":[{"x":111.48191438199856,"y":63.08402841937157},{"x":132.48025567384823,"y":63.08402841937157}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da7185358191631573","data":[{"x":111.48191438199856,"y":77.14150758466953},{"x":132.48025567384823,"y":77.14150758466953}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da36694145641926645","data":[{"x":111.48191438199856,"y":91.19898674996747},{"x":132.48025567384823,"y":91.19898674996747}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da08332047198623616","data":[{"x":111.48191438199856,"y":105.25646591526542},{"x":132.48025567384823,"y":105.25646591526542}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da5075417869365522","data":[{"x":111.48191438199856,"y":119.31394508056339},{"x":132.48025567384823,"y":119.31394508056339}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da6491827651659621","data":[{"x":112.58709023946433,"y":132.36731859119718},{"x":133.585431531314,"y":132.36731859119718}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"dp7564686579688207","type":"rectangle","data":{"p1":{"x":181.84479979217974,"y":33.964964434111536},"p2":{"x":202.10633469419184,"y":146.42479775649517}}},{"id":"da8696075699771535","data":[{"x":181.1079934023422,"y":49.02654925407362},{"x":189.94940026206837,"y":49.02654925407362},{"x":202.10633469419184,"y":49.02654925407362}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da343616438715983","data":[{"x":181.1079934023422,"y":63.08402841937157},{"x":202.10633469419184,"y":63.08402841937157}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da261937029824975","data":[{"x":181.1079934023422,"y":77.14150758466953},{"x":202.10633469419184,"y":77.14150758466953}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da27909409129600193","data":[{"x":181.1079934023422,"y":91.19898674996747},{"x":202.10633469419184,"y":91.19898674996747}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da07867044014771507","data":[{"x":181.1079934023422,"y":105.25646591526542},{"x":202.10633469419184,"y":105.25646591526542}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da6148243347915587","data":[{"x":181.1079934023422,"y":119.31394508056339},{"x":202.10633469419184,"y":119.31394508056339}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da021332501029793005","data":[{"x":182.21316925980796,"y":132.36731859119718},{"x":203.21151055165763,"y":132.36731859119718}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"dp9913964784881185","type":"rectangle","data":{"p1":{"x":208.3690203713583,"y":33.964964434111536},"p2":{"x":228.63055527337036,"y":146.42479775649517}}},{"id":"da9499189836639417","data":[{"x":207.63221398152072,"y":49.02654925407362},{"x":216.47362084124688,"y":49.02654925407362},{"x":228.63055527337036,"y":49.02654925407362}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da5091767964893957","data":[{"x":207.63221398152072,"y":63.08402841937157},{"x":228.63055527337036,"y":63.08402841937157}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da5413950068578494","data":[{"x":207.63221398152072,"y":77.14150758466953},{"x":228.63055527337036,"y":77.14150758466953}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da5823432492981727","data":[{"x":207.63221398152072,"y":91.19898674996747},{"x":228.63055527337036,"y":91.19898674996747}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da526604239684355","data":[{"x":207.63221398152072,"y":105.25646591526542},{"x":228.63055527337036,"y":105.25646591526542}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da6756120190135022","data":[{"x":207.63221398152072,"y":119.31394508056339},{"x":228.63055527337036,"y":119.31394508056339}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da7570672490014455","data":[{"x":208.73738983898647,"y":132.36731859119718},{"x":229.73573113083614,"y":132.36731859119718}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"dp6864065165229294","type":"rectangle","data":{"p1":{"x":237.10359266546834,"y":33.964964434111536},"p2":{"x":257.36512756748044,"y":146.42479775649517}}},{"id":"da28961443047696034","data":[{"x":236.36678627563077,"y":49.02654925407362},{"x":245.20819313535696,"y":49.02654925407362},{"x":257.36512756748044,"y":49.02654925407362}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da058129115088801475","data":[{"x":236.36678627563077,"y":63.08402841937157},{"x":257.36512756748044,"y":63.08402841937157}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da8444526197274174","data":[{"x":236.36678627563077,"y":77.14150758466953},{"x":257.36512756748044,"y":77.14150758466953}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da2375338698336804","data":[{"x":236.36678627563077,"y":91.19898674996747},{"x":257.36512756748044,"y":91.19898674996747}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da40260895008566056","data":[{"x":236.36678627563077,"y":105.25646591526542},{"x":257.36512756748044,"y":105.25646591526542}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da5819948029023745","data":[{"x":236.36678627563077,"y":119.31394508056339},{"x":257.36512756748044,"y":119.31394508056339}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da8997598430284909","data":[{"x":237.47196213309655,"y":132.36731859119718},{"x":258.4703034249462,"y":132.36731859119718}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"dp05941131784047338","type":"rectangle","data":{"p1":{"x":264.73298910211264,"y":33.964964434111536},"p2":{"x":284.99452400412474,"y":146.42479775649517}}},{"id":"da5501561722259058","data":[{"x":263.9961827122751,"y":49.02654925407362},{"x":272.83758957200126,"y":49.02654925407362},{"x":284.99452400412474,"y":49.02654925407362}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da2383270370780307","data":[{"x":263.9961827122751,"y":63.08402841937157},{"x":284.99452400412474,"y":63.08402841937157}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da21452046957488102","data":[{"x":263.9961827122751,"y":77.14150758466953},{"x":284.99452400412474,"y":77.14150758466953}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da9351436026039698","data":[{"x":263.9961827122751,"y":91.19898674996747},{"x":284.99452400412474,"y":91.19898674996747}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da8322349791998653","data":[{"x":263.9961827122751,"y":105.25646591526542},{"x":284.99452400412474,"y":105.25646591526542}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da7937067745605829","data":[{"x":263.9961827122751,"y":119.31394508056339},{"x":284.99452400412474,"y":119.31394508056339}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da9795295864350905","data":[{"x":265.10135856974085,"y":132.36731859119718},{"x":286.0996998615905,"y":132.36731859119718}],"head":"no","tail":"no","shaft":"-","mVer":1}],"settings":{"grid":true,"diagramHeight":302.29998779296875,"snapToOtherShapes":true}}]},{"id":"n0.8157475708500018","blocks":[],"style":null},{"id":"n0.9952180935752186","blocks":[]},{"id":"n0.1859510774886608","blocks":[],"style":null},{"id":"n0.022754700235529612","blocks":[],"style":null},{"id":"n0.8887157468951213","blocks":[],"style":null},{"id":"n0.1806774676610664","blocks":[]},{"id":"n0.3189872111783818","blocks":[],"style":null}],"pageSettings":{"pageSize":{"width":350,"height":1100}},"___version":2,"version":2,"av":1600,"delayRenderCache":{"av":1600,"map":{}}}

==> src/docs/2f92ee33-856a-4a82-b6ca-6fbdf139f0b9 <==
{"id":"r0.4251079482616569","lines":[{"id":"n0.665752554782286","blocks":[]},{"id":"n0.4834829444659675","blocks":[{"id":"n0.5307683728501813","text":"\\diagram","type":"composite","elements":{"de33588903072847676":{"id":"de33588903072847676","lines":[{"id":"n0.5439997934475511","blocks":[{"id":"n0.6549265240773969","text":"Programmable Fabric","style":{"fontSize":"\\scriptsize"}}]}],"shape":{"data":{"p":{"x":75,"y":74}},"anchor":"left-top"},"isTextMode":true},"de514618116099478":{"id":"de514618116099478","lines":[{"id":"n0.5826421798348669","blocks":[{"id":"n0.460376716273861","text":"FPGA Instance"}]}],"shape":{"data":{"p":{"x":47,"y":55}},"anchor":"left-top"},"isTextMode":true},"de5236748441099427":{"id":"de5236748441099427","lines":[{"id":"n0.7429411798117113","blocks":[{"id":"n0.8879189768196419","text":"Host CPU","style":{"fontSize":"\\scriptsize"}}]}],"shape":{"data":{"p":{"x":22,"y":87}},"anchor":"left-top"},"isTextMode":true},"de23016926915348135":{"id":"de23016926915348135","lines":[{"id":"n0.6779114278490614","blocks":[{"id":"n0.6295765597095233","text":"Remote User"}]}],"shape":{"data":{"p":{"x":66.72500610351562,"y":225.0500030517578}},"anchor":"center"},"isTextMode":true},"de6732908283163346":{"id":"de6732908283163346","lines":[{"blocks":[{"id":"n0.6846436291318648","text":"Data Center"}],"id":"n0.7921654899276858"}],"shape":{"data":{"p":{"x":58,"y":31}},"anchor":"left-top"},"isTextMode":true},"de6488941805358981":{"id":"de6488941805358981","lines":[{"id":"n0.4593308575030737","blocks":[{"id":"n0.6408369619569227","text":"⏲","style":{"fontSize":"\\Huge"}}]}],"shape":{"data":{"p":{"x":191,"y":96}},"anchor":"left-top"},"isTextMode":true},"de6790238935083176":{"id":"de6790238935083176","lines":[{"blocks":[{"text":"Programmable Fabric","style":{"fontSize":"\\scriptsize"},"id":"n0.4056537952800292"}],"id":"n0.18126308587713047"}],"shape":{"data":{"p":{"x":301,"y":74}},"anchor":"left-top"},"isTextMode":true},"de8044428232260089":{"id":"de8044428232260089","lines":[{"blocks":[{"text":"FPGA Instance","id":"n0.48603529855106"}],"id":"n0.28893802839963445"}],"shape":{"data":{"p":{"x":273,"y":56}},"anchor":"left-top"},"isTextMode":true},"de8367536791055977":{"id":"de8367536791055977","lines":[{"blocks":[{"text":"Host CPU","style":{"fontSize":"\\scriptsize"},"id":"n0.7774665767292886"}],"id":"n0.7307260032054181"}],"shape":{"data":{"p":{"x":248,"y":87}},"anchor":"left-top"},"isTextMode":true},"de02683481130212506":{"id":"de02683481130212506","lines":[{"blocks":[{"text":"Data Center","id":"n0.505581849059627"}],"id":"n0.3720930212350666"}],"shape":{"data":{"p":{"x":282,"y":30}},"anchor":"left-top"},"isTextMode":true},"de9887531689579374":{"id":"de9887531689579374","lines":[{"blocks":[{"text":"Programmable Fabric","style":{"fontSize":"\\scriptsize"},"id":"n0.3336889164691268"}],"id":"n0.8834729706007085"}],"shape":{"data":{"p":{"x":528,"y":75}},"anchor":"left-top"},"isTextMode":true},"de0951509646315657":{"id":"de0951509646315657","lines":[{"blocks":[{"text":"FPGA Instance","id":"n0.0026539926037416617"}],"id":"n0.6897756462866168"}],"shape":{"data":{"p":{"x":500,"y":57}},"anchor":"left-top"},"isTextMode":true},"de3613148998901209":{"id":"de3613148998901209","lines":[{"blocks":[{"text":"Host CPU","style":{"fontSize":"\\scriptsize"},"id":"n0.018295311887574384"}],"id":"n0.8354181565162403"}],"shape":{"data":{"p":{"x":475,"y":88}},"anchor":"left-top"},"isTextMode":true},"de10443289379945286":{"id":"de10443289379945286","lines":[{"blocks":[{"text":"Data Center","id":"n0.560723015667416"}],"id":"n0.9832913988447722"}],"shape":{"data":{"p":{"x":509,"y":31}},"anchor":"left-top"},"isTextMode":true},"de46105200720815775":{"id":"de46105200720815775","lines":[{"blocks":[{"id":"n0.912747798461571","text":"TDC","style":{"fontSize":"\\footnotesize"}}],"id":"n0.03970196850003049"}],"shape":{"data":{"p":{"x":555.8333129882812,"y":110}},"anchor":"left-top"},"isTextMode":true},"de27560740474990697":{"id":"de27560740474990697","lines":[{"blocks":[{"text":"⏲","style":{"fontSize":"\\Huge"},"id":"n0.2871385627594707"}],"id":"n0.7892853738950221"}],"shape":{"data":{"p":{"x":417,"y":97}},"anchor":"left-top"},"isTextMode":true},"de47481414144428336":{"id":"de47481414144428336","lines":[{"id":"n0.15174476357671596","blocks":[{"id":"n0.44224044732912626","text":"\\math-container","type":"composite","elements":{"mathValue":{"id":"n0.4945645046180279","lines":[{"id":"n0.563634696084793","blocks":[{"id":"n0.47062813564885475","text":"𝜖"}]}]}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"}}]}],"shape":{"data":{"p":{"x":433,"y":52}},"anchor":"left-top"},"isTextMode":true},"de6248569905417655":{"id":"de6248569905417655","lines":[{"id":"n0.5136350506176031","blocks":[{"id":"n0.7702842063613662","text":"⋙ "},{"id":"n0.9885716623937505","text":"\\math-container","type":"composite","elements":{"mathValue":{"id":"n0.3200162756969511","lines":[{"id":"n0.49036447485141754","blocks":[{"id":"n0.8523344447063029","text":"𝜖"}]}]}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"}}]}],"shape":{"data":{"p":{"x":199,"y":54}},"anchor":"left-top"},"isTextMode":true},"de8936718575125532":{"id":"de8936718575125532","lines":[{"id":"n0.3034009056753705","blocks":[{"id":"n0.851555053499426","text":"hours"}]}],"shape":{"data":{"p":{"x":194,"y":69}},"anchor":"left-top"},"isTextMode":true},"de6005013556487315":{"id":"de6005013556487315","lines":[{"blocks":[{"text":"hours","id":"n0.08034264067146513"}],"id":"n0.7681489421542299"}],"shape":{"data":{"p":{"x":421,"y":67}},"anchor":"left-top"},"isTextMode":true},"de6737067821073963":{"id":"de6737067821073963","lines":[{"id":"n0.4530925256579401","blocks":[{"id":"n0.2659234630087395","text":"1"}]}],"shape":{"data":{"p":{"x":27.166656494140625,"y":64.16665649414062}},"anchor":"center"},"isTextMode":true},"de2461202096530879":{"id":"de2461202096530879","lines":[{"blocks":[{"id":"n0.5126186360010856","text":"2"}],"id":"n0.028796422151300516"}],"shape":{"data":{"p":{"x":252,"y":64}},"anchor":"center"},"isTextMode":true},"de34509740104122444":{"id":"de34509740104122444","lines":[{"blocks":[{"id":"n0.006260676370431262","text":"3"}],"id":"n0.6071526797702459"}],"shape":{"data":{"p":{"x":479,"y":65}},"anchor":"center"},"isTextMode":true},"de5466804949478612":{"id":"de5466804949478612","lines":[{"blocks":[{"text":"Remote User","id":"n0.7211577979447164"}],"id":"n0.7072384161767078"}],"shape":{"data":{"p":{"x":295.7250061035156,"y":225.66668701171875}},"anchor":"center"},"isTextMode":true},"de2326906976987846":{"id":"de2326906976987846","lines":[{"blocks":[{"text":"Remote User","id":"n0.998387925902066"}],"id":"n0.3194936533211993"}],"shape":{"data":{"p":{"x":520.7250061035156,"y":226.66668701171875}},"anchor":"center"},"isTextMode":true},"de7915726721303712":{"id":"de7915726721303712","lines":[{"id":"n0.8227002094312497","blocks":[{"id":"n0.1666213576388379","text":"Victim Burn-in"}]}],"shape":{"data":{"p":{"x":167,"y":-1}},"anchor":"left-top"},"isTextMode":true},"de7885336556428892":{"id":"de7885336556428892","lines":[{"blocks":[{"id":"n0.11466285226192496","text":"Attack Phase"}],"id":"n0.1663909615371275"}],"shape":{"data":{"p":{"x":511,"y":-2}},"anchor":"left-top"},"isTextMode":true}},"connections":[],"intersections":{"id":"di826432440356249","items":[],"style":{}},"shapes":[{"id":"dp8882955946815936","type":"rectangle","data":{"p1":{"x":541,"y":147},"p2":{"x":590.3333129882812,"y":171}},"style":{"fillColor":[255,0,0,0.35]}},{"id":"dp9791105806599456","type":"rectangle","data":{"p1":{"x":82,"y":95},"p2":{"x":176.33331298828125,"y":176}}},{"id":"dp472213826890435","type":"circle","data":{"p1":{"x":93,"y":151},"p2":{"x":108.33331298828125,"y":166.33331298828125}}},{"id":"da9341008830493497","data":[{"x":106,"y":153},{"x":132.33331298828125,"y":153}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da33448278003712306","data":[{"x":132.33331298828125,"y":153},{"x":132.33331298828125,"y":160}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da5696093203922211","data":[{"x":125.33331298828125,"y":153},{"x":125.33331298828125,"y":160}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da06844957255827899","data":[{"x":119.16665649414062,"y":153},{"x":119.16665649414062,"y":160}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"dp6344189668157516","type":"rectangle","data":{"p1":{"x":88,"y":146},"p2":{"x":137.33331298828125,"y":170}},"style":{"fillColor":[0,255,0,0.14]}},{"id":"dp0035246497761196594","type":"square","data":{"p1":{"x":87,"y":102},"p2":{"x":113,"y":128}}},{"id":"dp21085747724715642","type":"square","data":{"p1":{"x":122,"y":103},"p2":{"x":135,"y":116}}},{"id":"dp7115128117752131","type":"square","data":{"p1":{"x":146,"y":144},"p2":{"x":163,"y":161}}},{"id":"dp44423681220770017","type":"square","data":{"p1":{"x":122.66665649414062,"y":129},"p2":{"x":135.66665649414062,"y":142}}},{"id":"dp8618086502964667","type":"square","data":{"p1":{"x":143,"y":103},"p2":{"x":169,"y":129}}},{"id":"da030264168221142085","data":[{"x":96,"y":129},{"x":96.33331298828125,"y":145}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da6410482474260685","data":[{"x":113.33331298828125,"y":111},{"x":121.33331298828125,"y":111}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da2162306014101809","data":[{"x":113.33331298828125,"y":121},{"x":142.33331298828125,"y":121}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da9546539620325721","data":[{"x":154.33331298828125,"y":129},{"x":154.33331298828125,"y":144}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da860459332248337","data":[{"x":137.33331298828125,"y":154},{"x":146.33331298828125,"y":154}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da3108173799324395","data":[{"x":134.33331298828125,"y":109},{"x":142.33331298828125,"y":109}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da2385445954730241","data":[{"x":136.33331298828125,"y":136},{"x":154.33331298828125,"y":136}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da2528723016057741","data":[{"x":95.33331298828125,"y":136},{"x":122.33331298828125,"y":136}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"dp9317791818356939","type":"rectangle","data":{"p1":{"x":22.33331298828125,"y":78},"p2":{"x":183.33331298828125,"y":182}}},{"id":"dp006273388624544296","type":"grid","data":{"p1":{"x":34,"y":109},"p2":{"x":62.33331298828125,"y":137}},"settings":{"cellSize":5,"cellBorderOnly":true}},{"id":"da5531741753724377","data":[{"x":59,"y":119},{"x":81.33331298828125,"y":118}],"head":"no","tail":"no","shaft":"2~","mVer":1},{"id":"dp18400887718120917","type":"rectangle","data":{"p1":{"x":20.45001220703125,"y":216.10000610351562},"p2":{"x":112.45001220703125,"y":233.10000610351562}}},{"id":"dp1885033227554046","type":"rectangle","data":{"p1":{"x":14.33331298828125,"y":51.999999999999986},"p2":{"x":190.33331298828125,"y":203}}},{"id":"da45530083466539106","data":[{"x":191,"y":96},{"x":239.33331298828125,"y":96}],"head":">","tail":"no","shaft":".","mVer":1},{"id":"da027249275186469468","data":[{"x":190,"y":154},{"x":239.33331298828125,"y":154}],"head":">","tail":"no","shaft":".","mVer":1},{"id":"dp0913415891516467","type":"rectangle","data":{"p1":{"x":308,"y":95},"p2":{"x":402.33331298828125,"y":176}}},{"id":"dp8056978713046292","type":"circle","data":{"p1":{"x":319,"y":151},"p2":{"x":334.33331298828125,"y":166.33331298828125}}},{"id":"da988411973259978","data":[{"x":332,"y":153},{"x":358.33331298828125,"y":153}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da5379265856681569","data":[{"x":358.33331298828125,"y":153},{"x":358.33331298828125,"y":160}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da8975363322271038","data":[{"x":351.33331298828125,"y":153},{"x":351.33331298828125,"y":160}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da15427155495621137","data":[{"x":345.1666564941406,"y":153},{"x":345.1666564941406,"y":160}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"dp732160858281035","type":"rectangle","data":{"p1":{"x":314,"y":146},"p2":{"x":363.33331298828125,"y":170}},"style":{"fillColor":[255,0,0,0.35]}},{"id":"dp9207360772000117","type":"square","data":{"p1":{"x":313,"y":102},"p2":{"x":339,"y":128}}},{"id":"dp860359961597269","type":"square","data":{"p1":{"x":348,"y":103},"p2":{"x":361,"y":116}}},{"id":"dp9569715596591231","type":"square","data":{"p1":{"x":372,"y":144},"p2":{"x":389,"y":161}}},{"id":"dp5584929701330967","type":"square","data":{"p1":{"x":348.6666564941406,"y":129},"p2":{"x":361.6666564941406,"y":142}}},{"id":"dp26049867610204835","type":"square","data":{"p1":{"x":369,"y":103},"p2":{"x":395,"y":129}}},{"id":"da1209788671137515","data":[{"x":322,"y":129},{"x":322.33331298828125,"y":145}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da13670720553201243","data":[{"x":339.33331298828125,"y":111},{"x":347.33331298828125,"y":111}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da24156445582798802","data":[{"x":339.33331298828125,"y":121},{"x":368.33331298828125,"y":121}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da022861968565462965","data":[{"x":380.33331298828125,"y":129},{"x":380.33331298828125,"y":144}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da261189108660537","data":[{"x":363.33331298828125,"y":154},{"x":372.33331298828125,"y":154}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da151679857444859","data":[{"x":360.33331298828125,"y":109},{"x":368.33331298828125,"y":109}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da9349476924815359","data":[{"x":362.33331298828125,"y":136},{"x":380.33331298828125,"y":136}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da8032280815678716","data":[{"x":321.33331298828125,"y":136},{"x":348.33331298828125,"y":136}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"dp558903319639338","type":"rectangle","data":{"p1":{"x":248.33331298828125,"y":78},"p2":{"x":409.33331298828125,"y":182}}},{"id":"dp3630768009368218","type":"grid","data":{"p1":{"x":260,"y":109},"p2":{"x":288.33331298828125,"y":137}},"settings":{"cellSize":5,"cellBorderOnly":true}},{"id":"da6656307885757022","data":[{"x":285,"y":119},{"x":307.33331298828125,"y":118}],"head":"no","tail":"no","shaft":"2~","mVer":1},{"id":"dp7784318799237794","type":"rectangle","data":{"p1":{"x":240.33331298828125,"y":51.999999999999986},"p2":{"x":416.33331298828125,"y":203}}},{"id":"dp3274433982883037","type":"rectangle","data":{"p1":{"x":535,"y":96},"p2":{"x":629.3333129882812,"y":177}}},{"id":"dp0216405891610868","type":"circle","data":{"p1":{"x":546,"y":152},"p2":{"x":561.3333129882812,"y":167.33331298828125}},"style":{"strokeType":"."}},{"id":"da3701541028868456","data":[{"x":559,"y":154},{"x":585.3333129882812,"y":154}],"head":"no","tail":"no","shaft":".","mVer":1},{"id":"da9297969026863256","data":[{"x":585.3333129882812,"y":154},{"x":585.3333129882812,"y":161}],"head":"no","tail":"no","shaft":".","mVer":1},{"id":"da2670362195493673","data":[{"x":578.3333129882812,"y":154},{"x":578.3333129882812,"y":161}],"head":"no","tail":"no","shaft":".","mVer":1},{"id":"da05916759556738693","data":[{"x":572.1666564941406,"y":154},{"x":572.1666564941406,"y":161}],"head":"no","tail":"no","shaft":".","mVer":1},{"id":"dp008517762859289513","type":"rectangle","data":{"p1":{"x":475.33331298828125,"y":79},"p2":{"x":636.3333129882812,"y":183}}},{"id":"dp6213925643830401","type":"grid","data":{"p1":{"x":487,"y":110},"p2":{"x":515.3333129882812,"y":138}},"settings":{"cellSize":5,"cellBorderOnly":true}},{"id":"da42062803432210916","data":[{"x":512,"y":120},{"x":534.3333129882812,"y":119}],"head":"no","tail":"no","shaft":"2~","mVer":1},{"id":"dp28987727702615995","type":"rectangle","data":{"p1":{"x":467.33331298828125,"y":52.999999999999986},"p2":{"x":643.3333129882812,"y":204}}},{"id":"dp7372384744351124","type":"rectangle","data":{"p1":{"x":555.8333129882812,"y":110},"p2":{"x":587.3333129882812,"y":132}}},{"id":"da7806140988612964","data":[{"x":497,"y":135},{"x":497.45001220703125,"y":217.10000610351562}],"head":"no","tail":"no","shaft":"2~","mVer":1},{"id":"da6525154483561981","data":[{"x":587,"y":118},{"x":601.3333129882812,"y":118}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da26515259852856776","data":[{"x":601.3333129882812,"y":118},{"x":601.3333129882812,"y":160}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da5596642481001085","data":[{"x":590.3333129882812,"y":160},{"x":601.3333129882812,"y":160}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da7110593032614494","data":[{"x":565.3333129882812,"y":132},{"x":565.3333129882812,"y":146}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da07162195183335351","data":[{"x":417,"y":97},{"x":465.33331298828125,"y":97}],"head":">","tail":"no","shaft":".","mVer":1},{"id":"da2782835953423911","data":[{"x":416,"y":154},{"x":465.33331298828125,"y":154}],"head":">","tail":"no","shaft":".","mVer":1},{"id":"dp978302834159117","type":"circle","data":{"p1":{"x":18,"y":55},"p2":{"x":36.33331298828125,"y":73.33331298828125}}},{"id":"dp3232093370173169","type":"circle","data":{"p1":{"x":242.83334350585938,"y":54.833343505859375},"p2":{"x":261.1666564941406,"y":73.16665649414062}}},{"id":"dp4394644751652187","type":"circle","data":{"p1":{"x":469.8333435058594,"y":55.833343505859375},"p2":{"x":488.1666564941406,"y":74.16665649414062}}},{"id":"da810901082345102","data":[{"x":270,"y":134},{"x":270.45001220703125,"y":216.10000610351562}],"head":"no","tail":"no","shaft":"2~","mVer":1},{"id":"da7335739469623208","data":[{"x":44,"y":134},{"x":44.45001220703125,"y":216.10000610351562}],"head":"no","tail":"no","shaft":"2~","mVer":1},{"id":"dp04942375238473662","type":"rectangle","data":{"p1":{"x":249.45001220703125,"y":216.71669006347656},"p2":{"x":341.45001220703125,"y":233.71669006347656}}},{"id":"dp9275901376686332","type":"rectangle","data":{"p1":{"x":474.45001220703125,"y":217.71669006347656},"p2":{"x":566.4500122070312,"y":234.71669006347656}}},{"id":"dp011909324839824542","type":"brace","settings":{"blockIntersection":true},"data":{"p1":{"x":413.75,"y":35},"p2":{"x":14.75,"y":35}}},{"id":"dp064408263092257","type":"brace","settings":{"blockIntersection":true},"data":{"p1":{"x":643.75,"y":35},"p2":{"x":468.75,"y":35}}}],"settings":{"grid":true,"diagramHeight":240.66668701171875}}]},{"id":"n0.8591809143615428","blocks":[],"style":null}],"pageSettings":{"pageSize":{"width":700}},"___version":2,"version":2,"av":960,"delayRenderCache":{"av":960,"map":{}}}

==> src/docs/b036b5a9-0370-48eb-a490-87d60af5ca5f <==
{"id":"r0.049527695018553364","lines":[{"id":"n0.9671014379546016","blocks":[]},{"id":"n0.564236306069992","blocks":[{"id":"n0.030955479974488442","text":"\\diagram","type":"composite","elements":{"de2947805792104964":{"id":"de2947805792104964","lines":[{"blocks":[{"text":"Burn-in","id":"n0.8697396940780221"}],"id":"n0.6575123926186367"}],"shape":{"data":{"p":{"x":127.66668701171875,"y":5.3499908447265625}},"anchor":"left-top"},"isTextMode":true},"de0225005826650182":{"id":"de0225005826650182","lines":[{"blocks":[{"text":"Test ","style":{"fontSize":"\\small"},"id":"n0.6784805367277018"}],"style":{"lineHeightEm":0.7,"align":"center"},"id":"n0.8256121606770583"},{"blocks":[{"text":"Routes","id":"n0.24106216742550945"}],"style":{"lineHeightEm":0.7,"align":"center"},"id":"n0.5548110300012191"}],"shape":{"data":{"p":{"x":155,"y":187.79998779296875}},"anchor":"center"},"isTextMode":true},"de9695018204355501":{"id":"de9695018204355501","lines":[{"blocks":[{"text":"Empty","id":"n0.45635531635706605"}],"style":{"lineHeightEm":0.7,"align":"center"},"id":"n0.0455760740617166"},{"blocks":[{"text":"Slices","id":"n0.6538597211981799"}],"style":{"lineHeightEm":0.7,"align":"center"},"id":"n0.46958146501783127"}],"shape":{"data":{"p":{"x":132.66668701171875,"y":74.79998779296875}},"anchor":"left-top"},"isTextMode":true},"de31303638063491446":{"id":"de31303638063491446","lines":[{"blocks":[{"text":"Burn","id":"n0.5731572520971563"}],"style":{"lineHeightEm":0.7,"textDirection":"rtl","align":"center"},"id":"n0.9720420535199036"},{"blocks":[{"text":"Values","id":"n0.06811171313027875"}],"style":{"lineHeightEm":0.7,"textDirection":"rtl","align":"center"},"id":"n0.37136973141006235"}],"shape":{"data":{"p":{"x":152.67130788167321,"y":263.29998779296875}},"anchor":"center"},"isTextMode":true},"de6096782936286815":{"id":"de6096782936286815","lines":[{"blocks":[{"id":"n0.2751230121817704","text":"Arithmetic Heavy"}],"id":"n0.37699397540295"}],"shape":{"data":{"p":{"x":294,"y":144.2999847412109},"skewX":0,"rotation":90},"anchor":"center"},"isTextMode":true},"de7745669410261978":{"id":"de7745669410261978","lines":[{"blocks":[{"id":"n0.941504557243634","text":"Arithmetic Heavy"}],"id":"n0.7143022342681319"}],"shape":{"data":{"p":{"x":14.725006103515625,"y":147.24998474121094},"skewX":0,"rotation":270},"anchor":"center"},"isTextMode":true}},"connections":[],"intersections":{"id":"di2581903923790777","items":[],"style":{}},"shapes":[{"id":"dp4008414294548498","type":"rectangle","data":{"p1":{"x":2,"y":3.199981689453125},"p2":{"x":306,"y":281.1999816894531}},"style":{"fillColor":"none"}},{"id":"dp06051614326550192","type":"rectangle","data":{"p1":{"x":41.66668701171875,"y":32.79998779296875},"p2":{"x":60,"y":144.79998779296875}}},{"id":"dp023884516519055654","type":"rectangle","data":{"p1":{"x":37,"y":152.79998779296875},"p2":{"x":273,"y":222.79998779296875}},"style":{"strokeType":".","strokeColor":[0,0,0,1],"fillColor":[0,0,255,0.4]}},{"id":"dp6942884342953544","type":"rectangle","data":{"p1":{"x":30.66668701171875,"y":28.79998779296875},"p2":{"x":282,"y":152.79998779296875}},"style":{"strokeType":".","fillColor":[255,0,0,0.4]}},{"id":"da32334653746552333","data":[{"x":143.66668701171875,"y":39.79998779296875},{"x":168,"y":39.79998779296875}],"head":"no","tail":"no","shaft":".","mVer":1},{"id":"da13458225114557854","data":[{"x":143.66668701171875,"y":65.79998779296875},{"x":168,"y":65.79998779296875}],"head":"no","tail":"no","shaft":".","mVer":1},{"id":"da9761532311636717","data":[{"x":143.66668701171875,"y":113.79998779296875},{"x":168,"y":113.79998779296875}],"head":"no","tail":"no","shaft":".","mVer":1},{"id":"da0950428949801807","data":[{"x":143.66668701171875,"y":135.79998779296875},{"x":168,"y":135.79998779296875}],"head":"no","tail":"no","shaft":".","mVer":1},{"id":"da06824239514941788","data":[{"x":142.66668701171875,"y":165.79998779296875},{"x":167,"y":165.79998779296875}],"head":"no","tail":"no","shaft":".","mVer":1},{"id":"da2602149903011892","data":[{"x":142.66668701171875,"y":208.79998779296875},{"x":167,"y":208.79998779296875}],"head":"no","tail":"no","shaft":".","mVer":1},{"id":"da9996036127879797","data":[{"x":41,"y":47.79998779296875},{"x":49,"y":47.79998779296875},{"x":60,"y":47.79998779296875}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da23246441788854166","data":[{"x":41,"y":61.79998779296875},{"x":60,"y":61.79998779296875}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da06963448781940662","data":[{"x":41,"y":75.79998779296875},{"x":60,"y":75.79998779296875}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da968150482775792","data":[{"x":41,"y":89.79998779296875},{"x":60,"y":89.79998779296875}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da485673634574743","data":[{"x":41,"y":103.79998779296875},{"x":60,"y":103.79998779296875}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da6465478034019958","data":[{"x":41,"y":117.79998779296875},{"x":60,"y":117.79998779296875}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da20337733751095177","data":[{"x":42,"y":130.79998779296875},{"x":61,"y":130.79998779296875}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"dp6434046438616922","type":"rectangle","data":{"p1":{"x":65.66668701171875,"y":32.79998779296875},"p2":{"x":84,"y":144.79998779296875}}},{"id":"da20412956468502408","data":[{"x":65,"y":47.79998779296875},{"x":73,"y":47.79998779296875},{"x":84,"y":47.79998779296875}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da8443163299457771","data":[{"x":65,"y":61.79998779296875},{"x":84,"y":61.79998779296875}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da5699622768253536","data":[{"x":65,"y":75.79998779296875},{"x":84,"y":75.79998779296875}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da3715126234263483","data":[{"x":65,"y":89.79998779296875},{"x":84,"y":89.79998779296875}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da43679377845788225","data":[{"x":65,"y":103.79998779296875},{"x":84,"y":103.79998779296875}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da9303538888341247","data":[{"x":65,"y":117.79998779296875},{"x":84,"y":117.79998779296875}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da3864013825933573","data":[{"x":66,"y":130.79998779296875},{"x":85,"y":130.79998779296875}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"dp16407328017809575","type":"rectangle","data":{"p1":{"x":91.66668701171875,"y":32.79998779296875},"p2":{"x":110,"y":144.79998779296875}}},{"id":"da5177727201146363","data":[{"x":91,"y":47.79998779296875},{"x":99,"y":47.79998779296875},{"x":110,"y":47.79998779296875}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da9065272131799244","data":[{"x":91,"y":61.79998779296875},{"x":110,"y":61.79998779296875}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da9281392996891762","data":[{"x":91,"y":75.79998779296875},{"x":110,"y":75.79998779296875}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da46757493734637856","data":[{"x":91,"y":89.79998779296875},{"x":110,"y":89.79998779296875}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da7804396471100992","data":[{"x":91,"y":103.79998779296875},{"x":110,"y":103.79998779296875}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da703090308869368","data":[{"x":91,"y":117.79998779296875},{"x":110,"y":117.79998779296875}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da13257768297841455","data":[{"x":92,"y":130.79998779296875},{"x":111,"y":130.79998779296875}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"dp43970631369270596","type":"rectangle","data":{"p1":{"x":116.66668701171875,"y":32.79998779296875},"p2":{"x":135,"y":144.79998779296875}}},{"id":"da5906004095631051","data":[{"x":116,"y":47.79998779296875},{"x":124,"y":47.79998779296875},{"x":135,"y":47.79998779296875}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da3085163036688019","data":[{"x":116,"y":61.79998779296875},{"x":135,"y":61.79998779296875}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da025359906864307225","data":[{"x":116,"y":75.79998779296875},{"x":135,"y":75.79998779296875}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da5042644044860115","data":[{"x":116,"y":89.79998779296875},{"x":135,"y":89.79998779296875}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da29294590598573067","data":[{"x":116,"y":103.79998779296875},{"x":135,"y":103.79998779296875}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da8766571134915934","data":[{"x":116,"y":117.79998779296875},{"x":135,"y":117.79998779296875}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da4723707094344708","data":[{"x":117,"y":130.79998779296875},{"x":136,"y":130.79998779296875}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"dp7209044032901816","type":"rectangle","data":{"p1":{"x":179.66668701171875,"y":32.79998779296875},"p2":{"x":198,"y":144.79998779296875}}},{"id":"da9658329767681283","data":[{"x":179,"y":47.79998779296875},{"x":187,"y":47.79998779296875},{"x":198,"y":47.79998779296875}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da7931568862083217","data":[{"x":179,"y":61.79998779296875},{"x":198,"y":61.79998779296875}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da07042332265656714","data":[{"x":179,"y":75.79998779296875},{"x":198,"y":75.79998779296875}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da9842917068228215","data":[{"x":179,"y":89.79998779296875},{"x":198,"y":89.79998779296875}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da24297020907174782","data":[{"x":179,"y":103.79998779296875},{"x":198,"y":103.79998779296875}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da9645728198988007","data":[{"x":179,"y":117.79998779296875},{"x":198,"y":117.79998779296875}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da573122787493737","data":[{"x":180,"y":130.79998779296875},{"x":199,"y":130.79998779296875}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"dp46156099152149765","type":"rectangle","data":{"p1":{"x":203.66668701171875,"y":32.79998779296875},"p2":{"x":222,"y":144.79998779296875}}},{"id":"da844056684422749","data":[{"x":203,"y":47.79998779296875},{"x":211,"y":47.79998779296875},{"x":222,"y":47.79998779296875}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da6524974170494219","data":[{"x":203,"y":61.79998779296875},{"x":222,"y":61.79998779296875}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da9786572891640838","data":[{"x":203,"y":75.79998779296875},{"x":222,"y":75.79998779296875}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da3280576844172617","data":[{"x":203,"y":89.79998779296875},{"x":222,"y":89.79998779296875}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da20880231685102835","data":[{"x":203,"y":103.79998779296875},{"x":222,"y":103.79998779296875}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da9443527029661267","data":[{"x":203,"y":117.79998779296875},{"x":222,"y":117.79998779296875}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da8227291192636622","data":[{"x":204,"y":130.79998779296875},{"x":223,"y":130.79998779296875}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"dp5232300299352364","type":"rectangle","data":{"p1":{"x":229.66668701171875,"y":32.79998779296875},"p2":{"x":248,"y":144.79998779296875}}},{"id":"da6508407268184639","data":[{"x":229,"y":47.79998779296875},{"x":237,"y":47.79998779296875},{"x":248,"y":47.79998779296875}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da3021809823083246","data":[{"x":229,"y":61.79998779296875},{"x":248,"y":61.79998779296875}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da3714560024858983","data":[{"x":229,"y":75.79998779296875},{"x":248,"y":75.79998779296875}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da2829902515493087","data":[{"x":229,"y":89.79998779296875},{"x":248,"y":89.79998779296875}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da19077512063407898","data":[{"x":229,"y":103.79998779296875},{"x":248,"y":103.79998779296875}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da12867734213373827","data":[{"x":229,"y":117.79998779296875},{"x":248,"y":117.79998779296875}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da9857414977732508","data":[{"x":230,"y":130.79998779296875},{"x":249,"y":130.79998779296875}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"dp1373649784065334","type":"rectangle","data":{"p1":{"x":254.66668701171875,"y":32.79998779296875},"p2":{"x":273,"y":144.79998779296875}}},{"id":"da17745677156218165","data":[{"x":254,"y":47.79998779296875},{"x":262,"y":47.79998779296875},{"x":273,"y":47.79998779296875}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da8566684094731759","data":[{"x":254,"y":61.79998779296875},{"x":273,"y":61.79998779296875}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da462915504249231","data":[{"x":254,"y":75.79998779296875},{"x":273,"y":75.79998779296875}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da07068191148822833","data":[{"x":254,"y":89.79998779296875},{"x":273,"y":89.79998779296875}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da802837104209035","data":[{"x":254,"y":103.79998779296875},{"x":273,"y":103.79998779296875}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da631078493640031","data":[{"x":254,"y":117.79998779296875},{"x":273,"y":117.79998779296875}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da07281654347366173","data":[{"x":255,"y":130.79998779296875},{"x":274,"y":130.79998779296875}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da21926311139663357","data":[{"x":51,"y":152.19998168945312},{"x":51,"y":235.19998168945312}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"strokeColor":[255,0,0,1],"thickness":3},"headScale":1},{"id":"da7088958436790096","data":[{"x":74,"y":153.19998168945312},{"x":74,"y":236.19998168945312}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"strokeColor":[0,255,0,1],"thickness":3}},{"id":"dp665155621094093","type":"generic-shape","data":{"p1":{"x":41.833343505859375,"y":235.19998168945312},"p2":{"x":60.166656494140625,"y":249.19998168945312}},"subType":"signal-ground","style":{"fillColor":[255,0,0,1],"strokeColor":[255,0,0,1],"thickness":3}},{"id":"da2947779449731148","data":[{"x":66.66668701171875,"y":237.19998168945312},{"x":81,"y":237.19998168945312}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"strokeColor":[0,255,0,1]}},{"id":"da39545445842187077","data":[{"x":101,"y":153.19998168945312},{"x":101,"y":236.19998168945312}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"strokeColor":[0,255,0,1],"thickness":3}},{"id":"da7707188983293655","data":[{"x":93.66668701171875,"y":237.19998168945312},{"x":108,"y":237.19998168945312}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"strokeColor":[0,255,0,1]}},{"id":"da06068126459269829","data":[{"x":126,"y":152.19998168945312},{"x":126,"y":235.19998168945312}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"strokeColor":[255,0,0,1],"thickness":3}},{"id":"dp6893444288088751","type":"generic-shape","data":{"p1":{"x":116.83334350585938,"y":235.19998168945312},"p2":{"x":135.16665649414062,"y":249.19998168945312}},"subType":"signal-ground","style":{"fillColor":[255,0,0,1],"strokeColor":[255,0,0,1],"thickness":3}},{"id":"da411380648685963","data":[{"x":189,"y":152.19998168945312},{"x":189,"y":235.19998168945312}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"strokeColor":[255,0,0,1],"thickness":3}},{"id":"dp9131196178867216","type":"generic-shape","data":{"p1":{"x":179.83334350585938,"y":235.19998168945312},"p2":{"x":198.16665649414062,"y":249.19998168945312}},"subType":"signal-ground","style":{"fillColor":[255,0,0,1],"strokeColor":[255,0,0,1],"thickness":3}},{"id":"da5067276455720623","data":[{"x":214,"y":152.19998168945312},{"x":214,"y":235.19998168945312}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"strokeColor":[255,0,0,1],"thickness":3}},{"id":"dp07460780262769728","type":"generic-shape","data":{"p1":{"x":204.83334350585938,"y":235.19998168945312},"p2":{"x":223.16665649414062,"y":249.19998168945312}},"subType":"signal-ground","style":{"fillColor":[255,0,0,1],"strokeColor":[255,0,0,1],"thickness":3}},{"id":"da11142652119277874","data":[{"x":238,"y":152.19998168945312},{"x":238,"y":235.19998168945312}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"strokeColor":[0,255,0,1],"thickness":3}},{"id":"da6517459637313696","data":[{"x":230.66668701171875,"y":236.19998168945312},{"x":245,"y":236.19998168945312}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"strokeColor":[0,255,0,1]}},{"id":"da9612030544040713","data":[{"x":265,"y":152.19998168945312},{"x":265,"y":235.19998168945312}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"strokeColor":[0,255,0,1],"thickness":3}},{"id":"da8388918085511583","data":[{"x":257.66668701171875,"y":236.19998168945312},{"x":272,"y":236.19998168945312}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"strokeColor":[0,255,0,1]}},{"id":"dp6472150138783904","type":"rectangle","data":{"p1":{"x":286,"y":19.249984741210938},"p2":{"x":301.45001220703125,"y":269.24998474121094}},"style":{"fillColor":"none"}},{"id":"dp3632167894127245","type":"rectangle","data":{"p1":{"x":7,"y":22.249984741210938},"p2":{"x":22.45001220703125,"y":272.24998474121094}},"style":{"fillColor":"none"}}],"settings":{"grid":false,"diagramHeight":302.29998779296875,"snapToOtherShapes":true}}]},{"id":"n0.8157475708500018","blocks":[],"style":null},{"id":"n0.9952180935752186","blocks":[]},{"id":"n0.1859510774886608","blocks":[],"style":null},{"id":"n0.022754700235529612","blocks":[],"style":null},{"id":"n0.8887157468951213","blocks":[],"style":null},{"id":"n0.1806774676610664","blocks":[]},{"id":"n0.3189872111783818","blocks":[],"style":null}],"pageSettings":{"pageSize":{"width":350,"height":1100}},"___version":2,"version":2,"av":1617,"delayRenderCache":{"av":1617,"map":{}}}
